Design and Experiments with LoCO AUV: A Low Cost Open-Source Autonomous Underwater Vehicle

In this paper we present LoCO AUV, a Low-Cost, Open Autonomous Underwater Vehicle. LoCO is a general-purpose, single-person-deployable, vision-guided AUV, rated to a depth of 100 meters. We discuss the open and expandable design of this underwater robot, as well as the design of a simulator in Gazebo. Additionally, we explore the platform's preliminary local motion control and state estimation abilities, which enable it to perform maneuvers autonomously. In order to demonstrate its usefulness for a variety of tasks, we implement a variety of our previously presented human-robot interaction capabilities on LoCO, including gestural control, diver following, and robot communication via motion. Finally, we discuss the practical concerns of deployment and our experiences in using this robot in pools, lakes, and the ocean. All design details, instructions on assembly, and code will be released under a permissive, open-source license.

==> fig/loco_3d.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/loco_final_top.jpg}
    \caption{LoCO AUV in CAD.}
    \label{fig:loco_3d}
    \vspace{-6mm}
\end{figure}

==> fig/loco_cameras.tex <==
\begin{figure}
    \centering
    \missingfigure[figwidth=0.49\textwidth]{Images from the 2 LoCO camera models.}
    \caption{}
    \label{fig:loco_cameras}
    \vspace{-6mm}
\end{figure}

==> src_tex/acknowledgements.tex <==
\section*{ACKNOWLEDGEMENTS}
